FaxPlainAC: A Fact-Checking Tool Based on EXPLAINable Models with HumAn Correction in the Loop

Fact-checking on the Web has become the main mechanism through which we detect the credibility of the news or information. Existing fact-checkers verify the authenticity of the information (support or refute the claim) based on secondary sources of information. However, existing approaches do not consider the problem of model updates due to constantly increasing training data due to user feedback. It is therefore important to conduct user studies to correct models' inference biases and improve the model in a life-long learning manner in the future according to the user feedback. In this paper, we present FaxPlainAC, a tool that gathers user feedback on the output of explainable fact-checking models. FaxPlainAC outputs both the model decision, i.e., whether the input fact is true or not, along with the supporting/refuting evidence considered by the model. Additionally, FaxPlainAC allows for accepting user feedback both on the prediction and explanation. Developed in Python, FaxPlainAC is designed as a modular and easily deployable tool. It can be integrated with other downstream tasks and allowing for fact-checking human annotation gathering and life-long learning.

==> 05ack.tex <==
\section{Acknowledgments}
This work is partially funded by \todo{@Avishek or @Koustav, could you please fill the proj. name and no. here? And do i need to mention ROXANNE since my salary is from that project?} and SoBigData (Grant agreement No. 654024).

==> related-work.tex <==
\section{Related Work}
\label{sec:related-work}

Ad-hoc retrieval is a classical task in information retrieval where there is precedence of classical probabilistic models based on query likelihood~\cite{lavrenko2017relevance} and BM25 proving hard to beat~\cite{robertson_bm25_2009}. 
In the last five years, neural models have been proposed to model semantic representations of the text~\cite{Shen2014a,dssm13,Shen2014b}, positional information~\citet{pacrr17,co_pacrr_wsdm18,pacrr_drmm_18}, local query-document interactions~\cite{KNRM17,Guo2016,matchpyramid16,Nie_ictir18,Nie_sigir_2018} or a combination of both~\cite{Mitra2017a}.
% We use a selection of these neural models for comparison (one from each model family). 
Recently, contextual models, using BERT, have proven to be superior than the above neural models.
The first work to use BERT was~\citet{macavaney2019contextualized:bertir:mpi} that used the contextualized embeddings of BERT as a replacement for word embeddings in existing document retrieval models (PACRR and KNRM). 
Closest to our work are models that try to address the variable-length limitation due to BERT's fixed input restriction either by passage-level labelling~\cite{dai_sigir_2019,wu_passage_webconf_2020} or sentence-wise labelling~\cite{lin_emnlp_2019}. \citet{dai_sigir_2019} proposed an approach to split documents into passages and then fine-tune BERT to obtain passage level relevance score(\doclabel). 
Such a document-labelling approach suffers from label noise because it assumes all passages of a relevant document are also relevant.
On the other hand,~\citet{lin_emnlp_2019} scored documents aggregating per-sentence relevance BERT scores using a cross-domain transfer model. 
Such a sentence-labelling approach has an unacceptably large inference time due to its sentence-level knowledge transfer.
We use it as a useful upper bound of the performance benefits due to contextual modelling of the entire document.
In this paper, our objective is to learn a selector and ranker in a joint manner to obviate heuristic design decisions relating to choice of passages for realizing a more effective and concise document representation.

Another line of work proposes weak supervision methods for training neural ranking architectures to learn from large-scale weak or noisy labels~\cite{Dehghani_sigir17,dehghani2018fidelityweighted,zhang_weak_wbconf_2020}. 
Other approaches inspired by the teacher-student paradigm~\cite{hinton2015distilling,xiao2015learning} attempt to infer better labels from noisy labels and use them to supervise the training of the network ~\cite{sukhbaatar2014training,veit2017learning}.
Although similar in spirit to our approach, our work judiciously selects evidence from the original training document and not creating more training labels using a selector model. 

\mpara{Select and predict models.}
Training models based on a subset of the input is broadly studied under feature selection in machine learning.
Different from classical feature selection, our aim is to select features from a document given a query. 
That is we want to dynamically select features (words, phrases and sentences) from a document based on the input query.
Such instance-wise feature selection has been explored in the machine learning literature~\citet{yoon2018:invase} however their applicability to modelling documents is limiting.
In computer vision, the selection phase is akin to using hard-attention models~\citet{malinowski2018learning} where a sub-image of a input image is chosen from downstream classification.
In NLP, simlar models are studied for ensuring interpretability by design~\citet{lei2016rationalizing,lehman2019inferring}. 
These works mainly differ in how they perform end-to-end training due to the explanation sampling step have been proposed subsequently. 
Common proposals for training include using REINFORCE~\cite{lei2016rationalizing}, actor-critic methods~\cite{yoon2018:invase}, or re-parameterization tricks~\cite{bastings2019interpretable}.
\citet{lehman2019inferring} uses a similar philosophy of decoupling rationale generator and predictor, albeit a slightly different architecture. 
~\citet{zhong2019fine} additionally used human annotations while learning from task supervision. 
However, we do not have any explicit training data to train the selector network and rather use the task supervision signal to update the parameters of the selector network. 

\mpara{Interpretable Models.}
For language tasks, there has been work on post-hoc analysis of already learned neural models by analyzing state activation~\cite{NIPS2013_5166, karpathy2015visualizing}~\cite{li2016understanding} or attention weights~\cite{bahdanau2014neural, cheng2016long, martins2016softmax, cui2016attention, xu2015multi, yang2016hierarchical}.
The attention weights learned as weights assigned to token representation are intended to describe rationales.
However, recently the faithfulness of interpreting model prediction with soft attention weights has been called into question \cite{wiegreffe2019attention, jain2019attention}. 
Specifically, contextual entanglement of inputs is non-trivial. The prediction model can still perform well even if the attention weights don't correlate with the (sub-)token weight as desired by humans.
Our approach for rationale based explanations differs in the type of architectures, objectives, and general nature of its utility. 






